Lost in Siting: The Hidden Carbon Cost of Inequitable Residential Solar Installations

The declining cost of solar photovoltaics (PV) combined with strong federal and state-level incentives have resulted in a high number of residential solar PV installations in the US. However, these installations are concentrated in particular regions, such as California, and demographics, such as high-income Asian neighborhoods. This inequitable distribution creates an illusion that further increasing residential solar installations will become increasingly challenging. Furthermore, while the inequity in solar installations has received attention, no prior comprehensive work has been done on understanding whether our current trajectory of residential solar adoption is energy- and carbon-efficient. In this paper, we reveal the hidden energy and carbon cost of the inequitable distribution of existing installations. Using US-based data on carbon offset potential, the amount of avoided carbon emissions from using rooftop PV instead of electric grid energy, and the number of existing solar installations, we surprisingly observe that locations and demographics with a higher carbon offset potential have fewer existing installations. For instance, neighborhoods with relatively higher black population have 7.4% higher carbon offset potential than average but 36.7% fewer installations; lower-income neighborhoods have 14.7% higher potential and 47% fewer installations. We propose several equity- and carbon-aware solar siting strategies. In evaluating these strategies, we develop Sunsight, a toolkit that combines simulation/visualization tools and our relevant datasets, which we are releasing publicly. Our projections show that a multi-objective siting strategy can address two problems at once; namely, it can improve societal outcomes in terms of distributional equity and simultaneously improve the carbon-efficiency (i.e., climate impact) of current installation trends by up to 39.8%.

==> 00-outline.tex <==
\newpage
\begin{enumerate}
{\color{blue}
    \item Introduction (1.5)
    \begin{itemize}
        \item results\/Carbon Offset\/CO vs Existing Quantile.png -- Currently Figure 1. Perhaps to similar to the Carbon Offset vs Existing installs plot.
        \item (If completed) Alternative to figure 1 -- continuous plot of carbon offset to proportion of panels owned by zips with Carbon Offset of x or lower (similar to CDF plot). 
    \end{itemize}
    
    \item Background and Motivation (0.75)
    \begin{enumerate}
        \item Residential Solar PV
        \item Solar and Carbon Offset Potential
        \item Incentives
        \item Inequities
    \end{enumerate}
}
    \item Carbon Offset Potential and Siting Analysis (2.5)
    \begin{enumerate}
        \item Problem Statement and Methodology
        \begin{enumerate}
            \item Problem Statement
            \begin{itemize}
                \item Results \/ Demographic Comparison \/ demo diff, both plots -- the bar plots of demographics against Carbon Offset Per Panel and Realized Potential (current figure 2)
                \item results\/Carbon Offset\/CO vs Existing  2.png -- Plot showing that upper quartile of carbon offsetters have disproportionately few panels. (current figure 4)
            \end{itemize}
            \item Datasets
        \end{enumerate}
        \item Solar Potential Analysis
            \begin{itemize}
                \item Sunlight vs Carbon Offset figure which was requested (in carbon offset folder, not current figure) 
                \item Energy Gen breakdown by State (current figure 5)
                \item We can replace this with all states instead of exemplar if we are removing that. 
            \end{itemize}
        \item Solar Siting Analysis
            \begin{itemize}
                \item Map of Carbon Offset by Zip (Figure 7)
                \item 2x3 maps (Figure 8)
            \end{itemize}
    \end{enumerate}
    \item Solar Siting Strategies (1.5)
    \begin{enumerate}
        \item The status quo
        \begin{itemize}
            \item Map of existing installs by zip (not current figure but already created)
            \item To be completed and  difficult to place in this outline (possibly in the equity impact section -- i.e. Geographic equity): Map of zip codes where each strategy places panels and how many it places (zip/ state granularity depending on what looks better)
        \end{itemize}
        \item Optimizing for Energy Efficiency
        \item Optimizing for Equity
        \item Optimizing for Carbon Efficiency
        \item Equitable Decarbonization
    \end{enumerate}
    \item Experimental Setup and Toolkit (0.5)
    \item Evaluation (2)
    \begin{enumerate}
        \item Energy Impact
        \begin{itemize}
            \item We could do a comparison between the greedy energy and equitable decarb strategies in a number of panels added vs Energy Gen plot but this would show the equitable strategy generates less power. 
        \end{itemize}
        \item Equity Impact
        \begin{itemize}
            \item To be polished, but completed: demographic analysis as in Figure 2, but after strategy is used.
        \end{itemize}
        \item Carbon Impact
        \begin{itemize}
            \item Unsure where to include: Projection of carbon offset of all strategies when building up to 2.5 million new panels (not current figure, in projections folder)
            \item To be completed: CO vs installs (like figure 1 or 4) but after using strategy.
        \end{itemize}
    \end{enumerate}
    \item Related Work (0.35)
    \item Conclusion (0.15)
\end{enumerate}



\section{Extra text}
\subsubsection{High Carbon Offset Regions}
In the introduction, in \autoref{fig:co_vs_existing_intro}, we show
that as the potential carbon offset per panel (at a ZIP code level) increases, so does the number of existing rooftop PV installations -- this trend continues until a sufficiently large potential carbon offset is reached, at which point the trend slows and eventually reverses.
% that as the potential carbon offset of ZIP codes increase so too does the number of rooftop panels installed in that ZIP code, that is, until sufficiently large potential carbon offset is reached, where the trend slows and eventually reverses. 
This implies that those areas that would offset the most carbon emissions with each new installations of rooftop PV have fewer existing panels than expected, and can be considered  ``underutilized''.

To examine this result in more detail, we plot each ZIP code's potential carbon offset (per panel) and existing installations as a scatter plot. We then separate the points into quartiles (4-quantiles instead of the 8-quantiles of \autoref{fig:co_vs_existing_intro}) and fit quadratic functions to minimize least squared error (LSE). After trying a variety of polynomial and exponential fits, we choose to report the quadratic fit as it and the linear fit were the only to not suffer from overfitting, though all fits exhibit the same basic trends.  \adaml{we should report the $R^2$ value for each quartile, either here or in caption}

These results are shown in \autoref{fig:co_vs_existing_main}. The most striking result is the abrupt change in trends between the 3rd and 4th quartile. In particular, we observe positive correlations between potential carbon offset and existing rooftop installations up until the 4th quartile, which has a negative correlation. There are a few possible explanations for this: 

\textbf{(1):} Due to the calculation of carbon offset, regions with many panels have low potential carbon offset \textit{now} because the grid is already substantially supplied using clean energy from existing rooftop PV. This is compelling, but insufficient because it fails to explain how there is a positive trend for the lower quartiles, which also source energy from other low-carbon sources. 

\textbf{(2):} ZIP codes in the 4th quartile with very few panels could be exemplars of the most influential demographics found in \autoref{Demos}. 
We find that this is partly true, but the ZIP codes with the highest carbon offsets (per panel) are not necessarily extreme examples of each individual 
%While this is partly true, we find that the ZIP codes with the highest carbon offset are not the most extreme in these 
demographics, but rather a combination of all. 
\rev{In \autoref{fig:state maps} we plot maps to further investigate this -- %we show that it can be seen that 
while there certainly is a trend, it is not a full explanation of this behavior.} \adaml{the flow with this sentence and the one previous is a bit off, maybe worth rewriting this second explanation.} 

\textbf{(3):} Both the potential carbon offset and the number of panels are correlated to region, states in particular, some of which do not prioritize low-carbon energy development and therefore have higher potential carbon offset due to their lack of clean energy, and likewise, a lack of rooftop PV. This is heavily supported by the findings of \autoref{Exemplars} and \autoref{oppurtunities} and is likely a substantial root cause.

\rev{We conclude that it is likely} \adaml{why do we conclude this?  after talking about the possible explanations we should give reasoning here.} that this \textit{carbon inefficiency} is in large part caused by regional differences in attitude towards clean energy, particularly rooftop solar installations. Further, such regions are more likely to skew towards states that tend to vote Republican and contain communities that have below-national-average incomes and above-national-average Black population proportions. % of low income, largely black, communities located in historically conservative states. 
We also conclude that this carbon inefficiency is caused in significant part, by the regions with the highest potential carbon offset. In what follows, we will determine which states seem to exhibit this inefficiency, postulate about the mechanisms that caused it, and propose mitigation strategies that could alleviate the most extreme of these inefficiencies.   


\newpage
\subsubsection{Correlated Demographics} \label{Demos}
As outlined in \autoref{sec:datasets}, we start with a pool of potential features within our dataset that \textit{may} correlate with solar installation trends, including racial demographics, median income, political alignment (via election results), and yearly average sunlight.

For each of these features, we split the dataset in two, grouping locations with a value of this feature \textit{above the national median} and a set of locations with feature value \textit{below the national median}, respectively. We then calculate the average carbon offset per viable panel and the average realized potential (current installations / viable installations) for both sides of the split as well as the entire dataset. 
We report the percent difference for carbon offset and existing installations when comparing the split subsets against the national average (i.e., the whole dataset).  Throughout the section, we report this difference at ZIP code and/or state-level granularities.







\smallskip
\noindent\textbf{Subsets of interest. \ }
Subsets of the population that are of interest are those with a carbon offset per panel significantly \textit{above} the national average and/or a realized potential significantly \textit{below} the national average. Any subset that simultaneously has an above-average carbon offset per panel and a below-average realized potential is henceforth termed ``underutilized'', since such subsets are prime targets for interventions to increase PV installations. 

Out of all of the demographic splits tested, three groups were found to be the most relevant -- i.e., these three demographics correlate well with the incidence of ``underutilized'' population subsets and/or areas of the United States. % as most relevant due to them meeting this criteria of being underutilized. 
The three demographics that correspond to underutilization are areas with an above-national-median Black population proportion, a below-national-median median income, and an above-national-median Republican voter proportion.
In states that meet any one of these criteria, the statewide numbers present a 
%Above-median Black population , below-median median income, and above-median Republican voter proportion states all had 
below-average realized potential and an above-average estimated carbon offset per panel. In \autoref{fig:demo_diff_state}, we report the values calculated for these three populations as well as their complements (e.g. below-median Black population proportion) and these same values for white population proportion as a baseline comparison.  

\smallskip
\noindent\textbf{Potential mechanisms of correlation. \ }
\autoref{fig:demo_diff_state} gives some interesting insights into the mechanism behind these disparities. Notably, it is interesting to see that the proportional differences for above-median Black proportion states are of a higher magnitude compared to those of below-median median income states, disproving the notion that this inequity for regions with high Black populations is solely caused by a correlation to low-income at a state-level. It is also worth noticing that while the states with above-national-median Republican voting records have the lowest realized potential out of all demographic splits tested, they have an average carbon offset per panel that is very close to the national average.%, \rev{which once again dispels the notion of a simple correlation.} \adaml{simple correlation with what?  I recommend just cutting this} 




We also conduct the same analysis at a ZIP code level granularity, for all of the features where data is available. We note that this does exclude political affiliation, however, because the precinct-level election data does not align to the ZIP code boundaries used for the carbon offset and realized potential values. %, these groups thus remain the same. 

At a ZIP code level, the demographics that have the highest proportional difference from the national average in carbon offset per panel and realized potential at match those from the state-level granularity reported in \autoref{fig:demo_diff_state}. 
In \autoref{fig:demo_diff_zip}, we report these ZIP code level proportional differences as percentages -- note that the reported figures for Republican voting are obtained by assigning each ZIP code the vote proportions of the state that contains it, because more granular data cannot be disaggregated along ZIP code boundaries.

% alongside the above-median Republican vote proportionortion group's proportional differences. 

Interestingly, at a ZIP code granularity it is no longer the case that the proportional differences of the above-median Black population proportion areas are strictly larger than the below-median median income areas. The average realized potential of the below-national-median median income group is lower than that of the above-national-median Black population group. Notably, the proportional differences for these two groups are lower in magnitude at a ZIP code granularity compared to the state-level granularity analysis.
% , the High Black Population group's proportional differences magnitude simply shrank more. 

From this pair of experiments, we continue with the following insights:
\begin{itemize}
    \item Areas (ZIP codes and/or states) with a high black population, low median income, and/or high Republican population are more likely to have a higher carbon offset per panel while also having fewer panels installed and can be considered ``underutilized''.
    % \item This underutilization is not explainable solely by a lack of suitable building locations. As shown in \autoref{fig:demo_diff_state} -- realized potential (i.e., the ratio of number of panels installed vs. the number of potentially viable roof locations for panels) is more inequitable than raw install count.
    \item A correlation with below-national-median median income does not sufficiently explain the underutilization of areas with an above-national-median Black population, at either a state or ZIP code level. Further, the disparity between these two at a state-level indicates that there is likely a racial disparity in how state- and local-level incentives/policies affect adoption of residential PV, aligning with prior findings.
    %design and who they effect in actuality.   
    \item It is likely that state-level policy differences largely account for these disparities, because political voting records are the most strongly negatively correlated feature for realized potential. In particular, this result raises the possibility that %it is likely that this is due to 
    a lack of effective state-level residential PV incentives result in this disparity, since the carbon offset per panel (which indirectly accounts for other low-carbon energy sources and policies excluding residential PV) correlation with political voting is less pronounced. We dive deeper into this phenomenon in \autoref{Exemplars}.
\end{itemize}








\newpage
 
 show
that as the potential carbon offset per panel (at a ZIP code level) increases, so does the number of existing rooftop PV installations -- this trend continues until a sufficiently large potential carbon offset is reached, at which point the trend slows and eventually reverses.
% that as the potential carbon offset of ZIP codes increase so too does the number of rooftop panels installed in that ZIP code, that is, until sufficiently large potential carbon offset is reached, where the trend slows and eventually reverses. 
This implies that those areas that would offset the most carbon emissions with each new installations of rooftop PV have fewer existing panels than expected, and can be considered  ``underutilized''.



To examine this result in more detail, we plot each ZIP code's potential carbon offset (per panel) and existing installations as a scatter plot. We then separate the points into quartiles (4-quantiles instead of the 8-quantiles of \autoref{fig:co_vs_existing_intro}) and fit quadratic functions to minimize least squared error (LSE). After trying a variety of polynomial and exponential fits, we choose to report the quadratic fit as it and the linear fit were the only to not suffer from overfitting, though all fits exhibit the same basic trends.  \adaml{we should report the $R^2$ value for each quartile, either here or in caption}

These results are shown in \autoref{fig:co_vs_existing_main}. The most striking result is the abrupt change in trends between the 3rd and 4th quartile. In particular, we observe positive correlations between potential carbon offset and existing rooftop installations up until the 4th quartile, which has a negative correlation. There are a few possible explanations for this: 

\textbf{(1):} Due to the calculation of carbon offset, regions with many panels have low potential carbon offset \textit{now} because the grid is already substantially supplied using clean energy from existing rooftop PV. This is compelling, but insufficient because it fails to explain how there is a positive trend for the lower quartiles, which also source energy from other low-carbon sources. 

\textbf{(2):} ZIP codes in the 4th quartile with very few panels could be exemplars of the most influential demographics found in \autoref{Demos}. 
We find that this is partly true, but the ZIP codes with the highest carbon offsets (per panel) are not necessarily extreme examples of each individual 
%While this is partly true, we find that the ZIP codes with the highest carbon offset are not the most extreme in these 
demographics, but rather a combination of all. 
\rev{In \autoref{fig:state maps} we plot maps to further investigate this -- %we show that it can be seen that 
while there certainly is a trend, it is not a full explanation of this behavior.} \adaml{the flow with this sentence and the one previous is a bit off, maybe worth rewriting this second explanation.} 

\textbf{(3):} Both the potential carbon offset and the number of panels are correlated to region, states in particular, some of which do not prioritize low-carbon energy development and therefore have higher potential carbon offset due to their lack of clean energy, and likewise, a lack of rooftop PV. This is heavily supported by the findings of \autoref{Exemplars} and \autoref{oppurtunities} and is likely a substantial root cause.

\rev{We conclude that it is likely} \adaml{why do we conclude this?  after talking about the possible explanations we should give reasoning here.} that this \textit{carbon inefficiency} is in large part caused by regional differences in attitude towards clean energy, particularly rooftop solar installations. Further, such regions are more likely to skew towards states that tend to vote Republican and contain communities that have below-national-average incomes and above-national-average Black population proportions. % of low income, largely black, communities located in historically conservative states. 
We also conclude that this carbon inefficiency is caused, in significant part, by the regions with the highest potential carbon offset. In what follows, we will determine which states seem to exhibit this inefficiency, postulate about the mechanisms that caused it, and propose mitigation strategies that could alleviate the most extreme of these inefficiencies.   

\newpage



{\color{brown}
\section*{temporary: moved here from section 4}

\subsubsection{Identifying Opportunities} \label{oppurtunities}
To summarize the experiments presented above, our results suggest that regions with a high Black population (as a proportion), low median income, and Republican voting tendencies correlate with low realized potential (i.e., few of the potential viable PV panel locations are populated) and high carbon offset (i.e., each PV panel displaces existing electricity generation that has high carbon intensity).
In this section, we examine the geographic location of these regions and identify patterns that suggest, e.g., which particular ZIP codes might be targeted to address this disparity.  

For example, at a state-level granularity, our analysis in \autoref{Exemplars} shows that Mississippi is an exemplar of both this issue and the predictive demographics.  At a ZIP code granularity (in \autoref{fig:co_per_cap_map}), we observe high carbon offset regions clustered towards the lower Midwest and upper Southeast regions of the US.


%\autoref{fig:co_per_cap_map} also reveals an interesting behavior. 
Though \autoref{fig:co_per_cap_map} visualizes carbon offset at a ZIP code granularity, there is a stark difference in values along some state lines. This is particularly noticeable in the Northeast between New York and Pennsylvania, corresponding to the boundary between the electric grids of the New York ISO (independent system operator) and the PJM interconnection (Pennsylvania-New Jersey-Maryland).
This division can be seen in \autoref{fig:state maps} as well, but the discernible state lines in the ZIP code granularity are more informative. There are also clear divides at some other state borders, such as Minnesota and California. 
These observations can be largely explained by the organization of electric grids in the United States, although different methods of reporting and data collection may also affect the reported carbon offset per panel.  Besides residential rooftop PV, these discrepancies also suggest differences in state-level energy policies and incentives that drive this issue of inequity and carbon inefficiency.

% This may be partially explained by different methods of data collection by ZIP code, or by discrepancies in how ZIP codes are distributed between different states, but this would not fully explain an order of magnitude difference across state lines. This result reinforces the notion that it is, in fact, a matter of State policy and incentives that drive this issue of inequity and carbon inefficiency.  

\subsubsection{Experimental Conclusions}
\adaml{some of the discussion here can either be cut or moved to section 3}


\rev{On its own, it is somewhat surprising to learn that there is an inequitable distribution of rooftop solar installations, in poor and black communities, to the degree that there is.} \adaml{this contradicts with what we already said in the related work / doesn't fit into the story of the paper -- I recommend not mentioning it}

In this United States-based study, it is interesting that much of the currently extant rooftop PV throughout the country seems to be biased towards regions that also have other forms of carbon-free energy available and/or do not receive substantial sunlight.  If the objective of building additional rooftop solar capacity within the US is to offset as many CO$_2$ emissions as possible, these issues of siting are paramount to efficiently leverage solar resources.

Furthermore, we find striking correlations between these observations and region characteristics such as racial demographics, income, and political affiliations.  Some of these correlations have been previously observed (e.g., that Black communities and low-income communities tend to have fewer rooftop PV installations), but our study particularly shines a light on the \textit{carbon inefficiency} that results from these distributional differences.

We postulate that the effects observed in the above sections are likely to be partially caused by differences in state/local policies towards clean energy development and rooftop PV in particular.  These policy differences may manifest in the form of e.g., fewer incentives for installation.  Correlations noticed with respect to voting patterns further suggest that regional attitudes and marketing efforts may also play a role -- for instance, electricity distributors and/or solar installation companies may choose to advertise in wealthier, white neighborhoods, possibly because of their ability and desire to install panels, or, perhaps, because of a racial bias. 
\adaml{ we didn't really talk about advertisement campaigns earlier so we should mention it when the median income correlation is discussed. }

% that we observed in the above sections, we find striking 
% Likewise, it is quite surprising how inefficiently placed a bulk of our rooftop solar installations are, in regions that are already supplied with clean energy or which don't receive substantial yearly sunlight.

% What is most concerning, however, is the degree to which these two issues are correlated, and, in fact, the likelihood that they are both due to state policies and advertisement campaigns which perpetuate this inequity and inefficiency. This may come in the form of fewer incentives either statewide, or in particular neighborhood. Likewise, 

Due to the correlation between carbon inefficiency and these demographics factors, it is likely that a combination of the above factors is at fault for perpetuating this inequity and inefficiency in terms of distribution of installations and carbon offset for each installation, respectively.  However, since efforts to expand rooftop PV in the United States can leverage both federal and state/local-level incentives, there are opportunities to address both the social distributional impacts and carbon inefficiency at the same time.  With the Inflation Reduction Act (IRA) of 2022, the US federal government increased the tax credit for residential PV to 30\% for ten years~\cite{EnergyGov:2023:ITC}.  Furthermore, the IRA also sets a precedent for \textit{targeted incentives}, such as special tax credits that incentivize industries and/or utilities to locate in low-income communities~\cite{TargetedIncentives}.  These suggest that one avenue to address the issues raised in the above sections is to design targeted incentives that e.g., maximize carbon offset per installation and/or target communities with few existing installations, which are more likely to be those regions exhibiting demographics discussed above.

%Luckily, there is an upside to proving this is a state issue. The federal government can give nationwide incentives, such as the 2022-2032 federal 30\% tax credit, that may allow these underutilized regions to become utilized. 
% Directed policy might even be created that could maximize carbon offset per dollar and, as an upshot, would mitigate the inequitable distribution of solar installations, for a time at least. 

However, as shown in \autoref{Exemplars}, we note that it is not necessarily clear that lowering the cost of rooftop PV is enough to fully address the disparities noticed in this paper.  Other factors, such as the prevailing electricity price in a region and cultural attitudes/trust towards new technologies, are likely equally important.  Disparities along racial lines may also result from implicit biases which cannot be easily ``fixed'' using top-down approaches such as federal-level monetary incentives.  Strategies to holistically address these issues must be the topic of future work. 

%it is not necessarily enough to lower the cost of installation. Likely it is the case that the energy price of a region largely affects the likelihood of adopting rooftop solar installations. 
% There is also, almost certainly, a racial bias that cannot be easily avoided simply through federal incentivization. Incentivization strategies and other approaches to solving these issues


}











\section{Exemplars (cutting from paper)?}
\subsubsection{Exemplar_States} \label{Exemplars}
To better demonstrate this problem at a state-level granularity, in this section we highlight five illustrative states in the US.  
These states were chosen as representative examples of
%We aimed for these states to be representative of the 
\textit{extremes} in terms of several variables of interest, including population racial composition, median income, political voting records, yearly average sunlight, electric generation sources, and state/local incentive schemes.  We detail our methodology below. 

To determine a representative group, we first calculate the average of each variable at the state level, finding the top and bottom five states for each (for racial composition, this process is done once for each census-reported group).
%(for racial composition this would be done over each racial group). 
Due to the heterogeneity in how state/local incentives are designed and implemented across the United States, there is no single useful quantification of incentive values.  As a proxy for these values, we used 
%For comparing local incentives it was not as obvious as there is not a singular quantification of these, instead we used 
an estimation of the expected cost of a 6 kW rooftop PV installation in each state \textit{after} federal and state incentives are applied. \adaml{we should cite where we got this estimate} We note that these estimate do not account for other rebates and incentives at the state/local level. \adaml{a rebate is a type of incentive, so this is confusing.  Perhaps we mean to say tax credit in the preceding sentence?}

In what follows, we describe the subset of five states that maximizes the number of extremes (i.e., top or bottom five across all states for any of the aforementioned variables):
\begin{itemize}
    \item \textbf{Delaware (DE):} Lowest clean energy generation proportion, below average incentives, moderate median income.
    \item \textbf{Massachusetts (MA):} Top 5 in median income, top 5 in solar generation proportion, but with highest cost per panel \cite{X}, and low average sunlight.
    \item \textbf{California (CA):} Top 5 in median income, top 5 in solar generation proportion, average cost per panel, and top 5 in yearly average sunlight. 
    \item \textbf{Mississippi (MI):} Bottom 5 in median income, top 5 in Black population proportion, top 5 in yearly average sunlight, average cost per panel (high when adjusting for income), and bottom 5 carbon-free energy proportion.
    \item \textbf{Texas (TX):} Top 5 in install count, below average cost per panel \cite{X}, top 5 in yearly average sunlight, moderate median income, and slightly high carbon-free energy (primarily wind). \adaml{install count wasn't mentioned earlier so mentioned it here is confusing.  Also, ``slightly high'' carbon-free energy is ambigious, need to be more concrete -- it's worth mentioning that it's mostly wind but we should say where it lies in the ranking.}
\end{itemize}
\adaml{missing cites in this list}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{results/Exemplar_States/energy_gen_breakdown_exemplar.png}
    \caption{Breakdown of the energy generation mix in the five exemplar states, sorted (left $\to$ right) by the solar generation proportion.}
    \label{fig:energy_breakdown}
\end{figure}

\begin{figure*}[t]
    \centering
  \subfloat[Black population proportion vs. carbon offset]{
	\begin{minipage}[c][0.5\width]{
	   0.33\textwidth}
	   \centering
	   \includegraphics[width=1\textwidth]{results/Exemplar_States/co_per_panel_vs_black_exemplar.png}
	\end{minipage}}
   \subfloat[Median income vs. carbon offset]{
	\begin{minipage}[c][0.5\width]{
	   0.33\textwidth}
	   \centering
	   \includegraphics[width=1\textwidth]{results/Exemplar_States/co_per_panel_vs_income_exemplar.png}
	\end{minipage}}
   \subfloat[Republican vote proportion vs. carbon offset]{
	\begin{minipage}[c][0.5\width]{
	   0.33\textwidth}
	   \centering
	   \includegraphics[width=1\textwidth]{results/Exemplar_States/co_per_panel_vs_republican_exemplar.png}
	\end{minipage}}
    \hfill
      \subfloat[Black population proportion vs. realized potential]{
	\begin{minipage}[c][0.5\width]{
	   0.33\textwidth}
	   \centering
	   \includegraphics[width=1\textwidth]{results/Exemplar_States/panel_util_vs_black_exemplar.png}
	\end{minipage}}
       \subfloat[Median income vs. realized potential]{
	\begin{minipage}[c][0.5\width]{
	   0.33\textwidth}
	   \centering
	   \includegraphics[width=1\textwidth]{results/Exemplar_States/panel_util_vs_income_exemplar.png}
	\end{minipage}}
       \subfloat[Republican vote proportion vs. realized potential]{
	\begin{minipage}[c][0.5\width]{
	   0.33\textwidth}
	   \centering
	   \includegraphics[width=1\textwidth]{results/Exemplar_States/panel_util_vs_republican_exemplar.png}
	\end{minipage}}
    \caption{Plotting trends in the carbon offset per panel and realized potential ($y$-axis) with respect to the Black proportion of the population, median income, and Republican voting percentage ($x$-axis) in each the exemplar states \adaml{worth increasing the size of each state label and reporting the $R^2$ value for each linear fit}}
    \label{fig:exemplar_trends}
\end{figure*}

In \autoref{fig:energy_breakdown}, we observe that the chosen states are diverse in their energy generation breakdown, with California and Massachusetts having significantly higher proportions of solar generation compared to the other states.  
% Furthermore, \autoref{fig:state maps} and \autoref{fig:exemplar_trends}  both visualize the diverse range of the subset chosen this way.
\adaml{it might be worth adding a table that gives concrete numbers for each of the (non-energy) variables in exemplar states.  Seems easier to explain than referring the reader to Figure 6 right before we talk about Figure 6 below}

In \autoref{fig:exemplar_trends}, we show relationships between the three underutilized demographics discussed in \autoref{Demos} and the average carbon offset per panel as well as the average realized potential in the chosen exemplar states. It is worth noting that these exemplar states were chosen independently of discovering the trends in \autoref{fig:exemplar_trends} -- thus, we make the following observations:
\begin{itemize}
    \item The five exemplar states are a representative set for \rev{the trends} \adaml{what trends?  better to be concrete to avoid confusing reader} discussed in this paper. \rev{Further, all six trends in \autoref{fig:exemplar_trends} are closely fit by a line, enforcing that this is a very predictable (and therefore treatable) issue using our three demographics.} \adaml{this is kind of subjective.  we should make a different claim here, something like ``the trends we observe in Fig X remain consistent across all exemplar states and all three main demographics of interest, suggesting that the issue of unrealized solar potential can be addressed by leveraging correlations with these demographics.}
    \item While both Massachusetts and California have built a sizable proportion of their possible rooftop solar adoption (higher realized potential) Texas has not, despite having a lower estimated cost per 6 kW installation. This suggests that either incentivizations outside of cost reduction play a large role in this phenomenon, or that the social/demographic makeup within the population influences these outcomes significantly.
\end{itemize}

==> 10-revision-detailed.tex <==
In what follows, we provide in-depth response to each of the reviewers' specific comments and reference the alterations made to address them.

\noindent \textbf{Review \#126A:} \textit{In other words, using carbon intensity to estimate “carbon offset potential” is a crude estimate at best, and may in some cases be entirely wrong. Unfortunately estimating true carbon offset potential is a very complex task that requires understanding local dispatch, market dynamics, and even flow of energy between interconnected regions. That would likely be beyond the scope of this paper, but at the very least, the fact that this is only an estimate should be made clear.}

\noindent \textbf{Revision: }
{\color{blue} We have made alterations, listed in \autoref{subsec:co-revision}, that we believe adequately explain the nature of the estimation used, as well as noting the shortcomings of such an estimation.} 

\noindent \textbf{Review \#126B: } \textit{The authors define carbon efficiency as the "amount of CO2 emissions prevented by each installation" (lines 167–169). However, there is no indication that they consider actual energy consumption and hence actual emissions in calculating this metric in the study. They rely on the raw "carbon offset potential" data without accounting for energy consumption, which could lead to overestimation or misrepresentation of carbon efficiency according to their definition. For carbon efficiency to be accurately gauged, factoring in actual energy consumption paired with a holistic view of the energy mix is essential, as this provides a more realistic and relevant view of CO2 mitigation.}

\noindent \textbf{Revision: }{\color{blue} We have highlighted the exact methodology of the Google Project Sunroof data (which uses the EPA eGrid
data in part of its calculation, specifically subregion CO2-equivalent non-baseload emission rates) and included an earlier reference to the methodology. We have also revised the section that describes the importance of the energy mix (\autoref{sec:background}, line 244) to clarify further.}

\smallskip

% {\color{blue}
% While concerns related to the carbon offset potential metric used as a major component of the paper are reasonable, with our revisions we have clarified the methodological details related to the accuracy of the method. The carbon offset metric is taken directly from Google’s Project Sunroof data set (which uses the EPA eGrid data in part of its calculation, specifically subregion CO2-equivalent non-baseload emission rates). The methodology is now described more explciitly in the paper as well as being reference earlier ([28] in the paper, line 377). We have also now included a more thorough description of the shortcomings of this estimation technique, particularly in its inability to account for timings of generation and demand. However, at the same time, we note that obtaining accurate carbon efficiency values is a formidable task, as mentioned by the reviewer. Further, we believe these obstacles do not significantly detract from the “broad strokes” findings of our work.}


\noindent \textbf{Review \#126A: }\textit{It's unclear what figure 1 is trying to communicate. If authors are trying to show the correlation between existing installations and carbon offset potential then the correlation coefficients or R values need to be shown.
}

\noindent \textbf{Revision: }{\color{blue}
To give a more meaningful analysis of \autoref{fig:co_vs_existing_intro} we calculated the Pearson correlation coefficient (PCC) for each of the quartiles. This is now reported in the caption of \autoref{fig:co_vs_existing_intro}. These new statistics add an additional nuance to the figure that was missing when only the quadratic fits were included. In particular, the PCC values show that while there is, in fact, a negative correlation only in the highest quartile, there is also a decreasing correlation as the estimated carbon offset increases between all quartiles. }

\smallskip

% \subsection{Optimization Formulation}
% % At the suggestion of Reviewer D we have made the formulation of solar siting problem as an optimization problem. \\ \\
% % \adaml{these two statements (above vs. below) contradict each other?}
% {\color{blue}
%  }

\noindent \textbf{Review \#126D: }\textit{Can the authors add more discussions on how to include a potential optimization problem formulation for deciding siting?
}

\noindent \textbf{Revision: }{\color{blue}
We have modified the description of the solar siting problem in \autoref{subsec:experiment} and the experimental setup description (in \autoref{sec:setup-toolkit}) to clarify the task and to assist future works formulating this problem as a multi-objective optimization problem.  We do not formalize the problem mathematically since the multi-objective nature of the problem is somewhat use-case specific -- however, we add a corresponding note to discuss the outstanding decisions (e.g., of the relative importances of each objective) that would facilitate an appropriate multi-objective optimization problem.

% We have altered the experimental setup description  to clarify the task, though we add a note that the formulation will be use-case specific if approached as an optmization problem. 
}

\smallskip


% \noindent \textbf{Review \#126D: }\textit{

% }
% \noindent \textbf{Revision: }{\color{blue}

% }

==> 9-revision-summary.tex <==
\subsection{Clarity of the Carbon Offset Estimation}\label{subsec:co-revision}
{\color{blue}
Following the reviewers' advice we have made the following changes to add clarity to the estimation of carbon offset used, the sources of those estimates, and the limitations thereof:
}
{\color{blue}
\begin{enumerate}
    \item Added a focus on timing of energy generation and demand in the initial description of Carbon Offset in \autoref{sec:background} alongside the mention of grid composition and dispatch. 
    \item Added a similar focus to the definition of Carbon Offset Potential in \autoref{sec:prob} where we define the problem and methodology.
    \item Made the origin of the Carbon Offset estimation data much more clear in \autoref{subsec:sunroof}. A fourth drawback of the dataset was also added explaining the weaknesses of the estimation techniques used. 
    \item Made particular mention of the "duck curve" timing problem which is referenced from a newly added citation \cite{Calero2022DuckCurveMI}.
\end{enumerate}}

\subsection{Existing Literature}
\noindent \textbf{Review \#126A: }\textit{A separate minor point: the related work section is quite short and typically for a 10-page paper there would be a longer discussion of the existing literature.}

\noindent \textbf{Revision: }{\color{blue} 
We have reviewed the literature related to rooftop PV and decarbonization.  In our revisions, we identified several additional related works that we have added as citations throughout the paper and in an expanded ``Related Work'' section.  While we believe that our work constitutes a contribution over the existing literature in the sense of the interactions that we study (e.g., between decarbonization goals and equity considerations), our expanded related work section improves our coverage of existing work, particularly amongst existing literature such as \citet{ElKontar2020} that have broadly considered the placement of PV panels or the decarbonization impacts of rooftop PV.  
}

% \adaml{ My preference is to find a few more papers (regardless of how directly related they actually are) that could fit into the related work and mention them here.  If we make this argument that we ``can't justify adding references'', the reviewers may interpret our response as lazy/standoffish -- it's not worth the risk IMO.}}

% \adaml{the shepherd's last point is  ``double check that the existing literature has been sufficiently covered and extend if needed'' so this detailed comment should go in the broader revision summary.}

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

